BioMistral-NLU: Towards More Generalizable Medical Language Understanding through Instruction Tuning

Large language models (LLMs) such as ChatGPT are fine-tuned on large and diverse instruction-following corpora, and can generalize to new tasks. However, those instruction-tuned LLMs often perform poorly in specialized medical natural language understanding (NLU) tasks that require domain knowledge, granular text comprehension, and structured data extraction. To bridge the gap, we: (1) propose a unified prompting format for 7 important NLU tasks, (2) curate an instruction-tuning dataset, MNLU-Instruct, utilizing diverse existing open-source medical NLU corpora, and (3) develop BioMistral-NLU, a generalizable medical NLU model, through fine-tuning BioMistral on MNLU-Instruct. We evaluate BioMistral-NLU in a zero-shot setting, across 6 important NLU tasks, from two widely adopted medical NLU benchmarks: BLUE and BLURB. Our experiments show that our BioMistral-NLU outperforms the original BioMistral, as well as the proprietary LLMs - ChatGPT and GPT-4. Our dataset-agnostic prompting strategy and instruction tuning step over diverse NLU tasks enhance LLMs' generalizability across diverse medical NLU tasks. Our ablation experiments show that instruction-tuning on a wider variety of tasks, even when the total number of training instances remains constant, enhances downstream zero-shot generalization.

==> sections/1_abstract.tex <==









%Giridhar abstract 
Large language models (LLMs) are pre-trained on large and diverse corpora and evaluated on different benchmarks. LLMs focused on medical language understanding have been evaluated only on a small subset of benchmarks, which are mainly focused on XX, XX. However, medical natural language understanding (NLU) involves more diverse tasks, including extracting granular information from medical text through entities and events, their relations, and longer context tasks, including sentence and document classification. Although these medical NLU tasks are widely performed, the effectiveness of LLMs has not been evaluated for (1) \textit{Generalizability} across diverse annotated medical phenomena and (2) \textit{Adaptability} across performing medical NLU tasks. In this work, we propose a novel framework that improves the generalizability and adaptability of LLMs for medical NLU tasks. Our framework includes (1) a comprehensive instruction-tuning corpus that encapsulates diverse annotated phenomena curated from existing open-source corpora and (2) a simple but efficient seq-seq framework that adapts LLMs to diverse medical NLU tasks. We evaluate our proposed system on common medical NLU benchmarks, Biomedical Language Understanding Evaluation (BLUE), and the Biomedical Language Understanding and Reasoning Benchmark (BLURB).  Our results show that our proposed model generalizes significantly better for BLUE and BLURB across 7 tasks and \textcolor{red}{14 out of 15} tasks but also exceeds GPT-4 in \textcolor{red}{7 out of 13} BLURB datasets evaluated. Our finding reveals that even with minimal prompt tuning, instruction tuning enhances LLMs' generalizability across medical NLU tasks.



% %Velvin abstract

% Previous research has demonstrated that following the finetuning phase across a diverse collection of instruction datasets, medical foundation large language models (LLMs) can generalize to new tasks. However, those instruction-tuned LLMs often perform poorly in specialized medical natural language understanding (NLU) tasks that require structured data extraction. This underperformance might be partially due to the focus on natural language generation (NLG) tasks which allow free-text and unconstrained outputs during the instruction-tuning phase. Recognizing the lack of comprehensive studies on adapting foundation LLMs for medical NLU tasks, we proposed a unified format for medical NLU and developed a specialized instruction-tuning dataset, MNLU-Instruct, targeting key medical NLU tasks. We finetuned the BioMistral-7B-DARE model on this dataset and created a new variant, BioMistral-NLU. We evaluated BioMistral-NLU performance against two public medical NLU benchmarks, BLURB and BLUE. Our results show that our proposed finetuned model, BioMistral-NLU, not only outperforms the original BioMistral-7B-DARE across 7 tasks and \textcolor{red}{14 out of 15} datasets but also exceeds GPT-4 in \textcolor{red}{7 out of 13} BLURB datasets evaluated. Our finding reveals that even with minimal prompt tuning, instruction tuning enhances LLMs' generalizability across medical NLU tasks.
% %However, those simplistic prompts fail to capture all nuances, which underscores the need for more detailed task instructions or annotated data as examples for medical NLU system development.
% We plan to release our data and code following the acceptance of this manuscript.
% % downstream applications such as fact-based evaluation?

==> sections/2_introduction.tex <==





\begin{figure}[h]
\centering
\includegraphics[width=7cm]{figures/system.jpg}
\caption{ Instruction-tuning dataset (MNLU-Instruct), system development, and downstream evaluation  for BioMistral-NLU.}\label{fig:system} 
\end{figure}

%giridhar Intro

Large Language Models (LLMs) have been trained and evaluated on tasks across different domains\cite{chung2022scaling,chowdhery2023palm,touvron2023llama}. LLMs specialized in the medical domain have shown great performance across various tasks such as medical exams  \cite{singhal2023large}, common sense reasoning  \cite{labrak2024biomistral, han2023medalpaca} showing in-depth domain knowledge and logical reasoning ability \cite{nori2023capabilities}, and diagnostic reasoning \cite{saab2024capabilities}.
Additionally, the GPT-4 model has been shown to generalize well for the medical domain \cite{}. 
LLMs, however, there is limited work studying the models for widely performed medical natural language understanding (MNLU) tasks such as named-entity and relation extraction  \cite{xie2024me, hu2023zero, ramachandran-etal-2023-prompt} and sentence classification  \cite{chen2024evaluating}. 

In this work, we study the \textit{generalizability} and the \textit{adaptability} of LLMs for medical NLU. Fimprove the generalizability of LLMs


Despite the improvements, the performance gap between the generalized BioMistral-7B-DARE and the in-domain fine-tuned systems highlights the complexities of many NLU tasks that cannot be captured by simplistic prompts. This observation underscores the need for more detailed task instructions or annotated data as examples for medical NLU system development.


%old intro
Finetuning large language models (LLMs) on a diverse collection of instruction-following datasets enables LLMs to generalize across a wide range of new tasks \cite{chung2022scaling,chowdhery2023palm,touvron2023llama}. 
Following this instruction finetuning phase, medical foundation LLMs \cite{zhang2024data, saab2024capabilities} have demonstrated great performance in various medical tasks, which requires in-depth domain knowledge and logical reasoning ability  \cite{nori2023capabilities}, such as medical exams  \cite{singhal2023large}, common sense reasoning  \cite{labrak2024biomistral, han2023medalpaca} and diagnostic reasoning \cite{saab2024capabilities}. %, without task-specific training
Despite their superior generalizability in some areas, instruction-tuned LLMs often underperform smaller-scale, finetuning-based language models, in some specialized medical natural language understanding (NLU) tasks. These NLU tasks involve extracting textual information into structured formats \cite{patel2021deep}, such as named-entity and relation extraction  \cite{xie2024me, hu2023zero, ramachandran-etal-2023-prompt} and sentence classification  \cite{chen2024evaluating}. The performance gap may be because the current foundation LLMs' instruction-tuning phase focuses primarily on natural language generation (NLG) tasks that allow for free-text, unconstrained outputs \cite{chung2022scaling}. Although many NLG tasks require complex logical reasoning, these skills do not directly translate into the nuanced NLU tasks, such as recognizing named entity labels and classifying the input sentences into constrained categories.

To the best of our knowledge, no comprehensive study has yet explored adapting LLMs specifically for medical NLU. To bridge this gap, we propose a unified format for medical NLU and construct an instruction-tuning dataset focused on 8 important medical NLU tasks (MNLU-Instruct). We finetuned BioMistral-7B-DARE \cite{labrak2024biomistral} on MNLU-Instruct, resulting in a new model variant we call BioMistral-NLU. To assess the model's generalizability, we evaluate BioMistral-NLU under a zero-shot setting using two public medical BLUE benchmarks: (1) the Biomedical Language Understanding and Reasoning Benchmark (BLURB) \cite{gu2021domain} and (2) the Biomedical Language Understanding Evaluation benchmark (BLUE) \cite{peng2019transfer} with minimum prompt-tuning. In our evalutation, BioMistral-NLU outperforms the original BioMistral-7B-DARE in 14 of the 15 datasets, and GPT-4 in \textcolor{red}{7 out of 13} tasks. Our result demonstrated that instruction-tuning on diverse medical NLU tasks using our unified format is an effective approach to improving the LLMs' generalizability. Despite the improvements, the performance gap between the generalized BioMistral-7B-DARE and the in-domain fine-tuned systems highlights the complexities of many NLU tasks that cannot be captured by simplistic prompts. This observation underscores the need for more detailed task instructions or annotated data as examples for medical NLU system development.

%This approach also offers the potential to replace traditional in-domain finetuning methods, and thus reduce the associated annotation and system development costs.

% We can write a similar contribution statement as InstructUIE: https://arxiv.org/pdf/2304.08085
% 1. We propose an end-to-end framework for universal information extraction – InstructUIE, which leverages natural language instructions to guide large language models for IE tasks.
% 2. We introduce IE INSTRUCTIONS, a benchmark of 32 diverse information extraction datasets in
% a unified text-to-text format with expert-written instructions.
% 3. Experimental results demonstrate that InstructUIE achieves comparable performance to Bert in a supervised setup. Notably, our method significantly outperforms the current state-of-theart and GPT-3.5 in a zero-shot setup.


==> tables/NER_relaxed.tex <==
\begin{table}[H]
\centering
\small
\resizebox{0.5\textwidth}{!}{%
\begin{tabular}{llccc}
\hline
\multirow{2}{*}{\textbf{Dataset}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}\# test\\ instances\end{tabular}}} & \multicolumn{1}{c|}{\textbf{BERT-SFT}} & \multicolumn{2}{c}{\textbf{BioMistral-NLU}} \\ \cline{3-5} 
 &  & \multicolumn{2}{c|}{\textbf{Entity-level F1}} & \textbf{Relaxed F1} \\ \hline
BC2GM & 6,322 & 84.5 & \multicolumn{1}{c|}{61.5} & 86.9 \\
BC5-chemical & 5,385 & 93.3 & \multicolumn{1}{c|}{89.9} & 92.7 \\
BC5-disease & 4,424 & 85.6 & \multicolumn{1}{c|}{67.0} & 85.7 \\
NCBI-disease & 955 & 89.1 & \multicolumn{1}{c|}{61.8} & 82.3 \\
JNLPBA & 8,657 & 79.1 & \multicolumn{1}{c|}{64.4} & 74.4 \\ \hline
Macro average & - & 86.3 & \multicolumn{1}{c|}{68.9} & 84.4 \\ \hline
\end{tabular}
}
\setlength{\belowcaptionskip}{-5pt}
\caption{F1 scores on unseen NER datasets under different evaluation criteria. }
\label{tab:ner_relaxed}
\end{table}



==> tables/instruction_tuning_details.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[h]
\small
\resizebox{\textwidth}{!}{%
\begin{tabular}{llrl}
\hline
\textbf{Task} & \textbf{dataset} & \textbf{\# instances} & \textbf{Labels} \\ \hline
\multirow{16}{*}{NER} & i2b2 2006DeID & 5,608 & Location, ID, Date, Hospital, Doctor, Contact, Name, Age \\ \cline{2-4}
 & i2b2 2011 & 25,689 & Person, Treatment, Test, Problem \\ \cline{2-4}
 & i2b2 2012 & 7,446 & \begin{tabular}[c]{@{}l@{}}Test, Problem, Frequency, Time, Date, Occurrence, Treatment,\\ Duration, Clinical department\end{tabular} \\ \cline{2-4}
 & i2b2 2014 & 52,462 & ID, Contact, Age, Name, Location, Profession, Date \\ \cline{2-4}
 & GENIA & 15,023 & RNA, DNA, Cell type, Protein, Cell line \\ \cline{2-4}
 & linnaeus & 11,935 & Species \\ \cline{2-4}
 & tmVar & 5,351 & \begin{tabular}[c]{@{}l@{}}Cell Line, SNP, Gene, Protein Mutation, Protein Allele, Species\\ DNA Allele, DNA Mutation, Other Mutation, Acid Change,\end{tabular} \\ \cline{2-4}
 & DrugProt & 17,274 & \begin{tabular}[c]{@{}l@{}}Organism Taxon, Disease Or Phenotypic Feature, Cell Line, \\ Gene Or Gene Product, Sequence Variant, Chemical\end{tabular} \\ \cline{2-4}
 & BioRed & 13,706 & Chemical, Gene \\ \cline{2-4}
 & GNorm & 4,006 & Family Name, Domain Motif, Gene \\ \cline{2-4}
 & NLM-Gene & 5,048 & \begin{tabular}[c]{@{}l@{}}Gene, Gene reference into function (function of a gene), Domain,\\ Steroidogenic acute regulatory protein (a protein coding gene)\end{tabular} \\ \cline{2-4}
 & ClinicalIE\_Med & 105 & Route, Duration, Reason, Dosage, Frequency, Medication \\ \cline{2-4}
 & ClinicalIE\_Status & 105 & Neither medications, Discontinued medications, Active medications \\ \cline{2-4}
 & BC4CHEMD & 30,682 & Chemical \\ \cline{2-4}
 & PubMed PICO & 1,961 & Species, Comparator, Outcome, Intervention, Strain, Induction \\ \cline{2-4}
 & PICO-Data & 36,224 & Participants, Intervention, Outcome \\ \hline
\multirow{3}{*}{EE} & i2b2 2009 & 117,446 & Medication (Dosage, Route, Frequency, Duration, Reason, Context) \\ \cline{2-4}
 & i2b2 2018 & 155,716 & Drug, ADE (Strength, Frequency, Reason, Form, Route, Dosage) \\ \cline{2-4}
 & n2c2 2022 & 36,359 & \begin{tabular}[c]{@{}l@{}}Alcohol, Drug, Tobacco, Employment, Living \\ (time, duration, history, type, amount, frequency)\end{tabular} \\ \hline
\multirow{6}{*}{DC} & i2b2 2006Smoke & 398 & Current smoker/Past smoker/Non-smoker/Unknown \\ \cline{2-4}
 & i2b2 2008 & 17,242 & 10 obesity commodities (Asthma, Depression, ...) \\ \cline{2-4}
 & n2c2 2018 & 2,626 & Different selection criteria for 13 cohorts (Abdominal, English, ...) \\ \cline{2-4}
 & 2024 SemEval2 & 1,700 & Adverse Events, Eligibility, Results, Intervention \\ \cline{2-4}
 & TrialStop & 3,747 & 17 reasons to stop a study (Study staff moved, Another study, ...) \\ \cline{2-4}
 & MTSamples & 3,206 & 48 medical specialties or domains (Bariatrics, Nephrology, ...) \\ \hline
\multirow{5}{*}{RE} & i2b2 2011 & 25,689 & Refers to \\ \cline{2-4}
 & i2b2 2012 & 7,446 & \begin{tabular}[c]{@{}l@{}}Ends by, Happens during, Happens before and overlap, Begins by,\\ Happens before, Happens simultaneously with, Happens after, \\ Overlaps with,\end{tabular} \\ \cline{2-4}
 & EUADR & 318 & Gene-disease association \\ \cline{2-4}
 & DrugProt & 35,624 & \begin{tabular}[c]{@{}l@{}}Antagonist, Agonist, Indirect upregulator, Part of, Agonist activator,\\ Substrate, Activator, Inhibitor, Direct regulator, Agonist inhibitor, \\ Product of, Substrate product of, Indirect downregulator\end{tabular} \\ \cline{2-4}
 & BioRed & 4,328 & \begin{tabular}[c]{@{}l@{}}Drug interaction, Positive correlation, Cotreatment, Comparison, \\ Bind, Conversion, Association, Negative correlation\end{tabular} \\ \hline
\multirow{3}{*}{NLI} & Multi-NLI & 785,404 & Entailment, Contradiction, Neutral \\ \cline{2-4}
 & SNLI & 1,098,734 & Entailment, Contradiction, Neutral \\ \cline{2-4}
 & BioNLI & 23,704 & Entailment, Contradiction, Neutral \\ \hline
STS & SIS-B & 11,018 & 6 similarity scales \\ \hline
\multirow{3}{*}{NLG} & PubMedSum & 1,407 & Article summarization \\ \cline{2-4}
 & CDSR & 436 & Article simplication \\ \cline{2-4}
 & AciDemo & 204 & Dialogue to note summarization \\ \hline
\end{tabular}
}
\setlength{\belowcaptionskip}{-5pt}
\caption{Task labels and number of instances in the MNLU-Instruct datasets. For EE tasks, labels inside () refer to event arguments. }
\label{tab:instruction-tuing_details}
\end{table}

==> tables/instruction_tuning_v1.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[h]
\small
\resizebox{\textwidth}{!}{%
\begin{tabular}{lll}
\hline
\textbf{Category} & \textbf{Task} & \textbf{Datasets} \\ \hline
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Token \\ classification\end{tabular}} & NER & \begin{tabular}[c]{@{}l@{}}i2b2 2006DeID  \cite{uzuner2007evaluating}, i2b2 2011Coreference  \cite{uzuner2012evaluating},\\ i2b2 2012Temporal  \cite{sun2013evaluating}, i2b2 2014 DeID  \cite{stubbs2015annotating}, \\ GENIA \cite{yu2020named}, linnaeus \cite{kocaman2021biomedical}, tmVar \cite{wei2018tmvar}, \\ DrugProt \cite{miranda2023overview}, BioRed \cite{luo2022biored},\\ GNorm \cite{morgan2008overview}, NLM-Gene \cite{islamaj2021nlm}, \\ ClinicalIE \cite{agrawal2022large}, BC4CHEMD \cite{kocaman2021biomedical},\end{tabular} \\ \cline{2-3} 
 & PICO & PubMed PICO  \cite{jin2018pico}, PICO-Data  \cite{nguyen2017aggregating} \\ \hline
\begin{tabular}[c]{@{}l@{}}Token \& \\ sequence\\ classification\end{tabular} & \begin{tabular}[c]{@{}l@{}}Event \\ extraction\end{tabular} & \begin{tabular}[c]{@{}l@{}}i2b2 2009Medication \cite{uzuner2010extracting}, i2b2 2018ADE  \cite{henry20202018}, \\ n2c2 2022SDoH \cite{lybarger20232022},\end{tabular} \\ \hline
\multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}Sequence\\ classification\end{tabular}} & \begin{tabular}[c]{@{}l@{}}Document\\ classification\end{tabular} & \begin{tabular}[c]{@{}l@{}}i2b2 2006Smoking \cite{uzuner2008identifying}, i2b2 2008Obesity \cite{uzuner2009recognizing}, \\ n2c2 2018  \cite{stubbs2019cohort}, 2024 SemEval Task 2  \cite{jullien2024semeval}, \\ TrialStop \cite{razuvayevskaya2023clinical}, MTSamples  \cite{MTSample}\end{tabular} \\ \cline{2-3} 
 & RE & \begin{tabular}[c]{@{}l@{}}i2b2 2011Coreference  \cite{uzuner2012evaluating}, i2b2 2012Temporal  \cite{sun2013evaluating}, \\ EUADR \cite{VANMULLIGEN2012879}, DrugProt \cite{miranda2023overview}, \\ BioRed \cite{luo2022biored}\end{tabular} \\ \cline{2-3} 
 & NLI & BioNLI  \cite{bastan2022bionli}, SNLI  \cite{bowman2015large}, Multi-NLI \cite{N18-1101} \\ \hline
\begin{tabular}[c]{@{}l@{}}Sequence\\ regression\end{tabular} & STS & SIS-B  \cite{wang2018glue} \\ \hline
NLG & Summarization & PubMedSum  \cite{cohan-etal-2018-discourse}, CDSR  \cite{guo2021automated}, AciDemo \cite{yim2023aci} \\ \hline
\end{tabular}
}
\caption{Publicly available medical datasets used in the instruction-tuning phase.}
\label{tab:instruction-tuing}
\end{table}



==> tables/results_withBERT.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[H]
\resizebox{\textwidth}{!}{%
% \renewcommand{\arraystretch}{0.4}\textbf{\begin{tabular}[c]{@{}c@{}}BERT-FT\\ \tiny \cite{peng2019transfer} \\ \tiny \cite{gu2021domain} \end{tabular}}
% \renewcommand{\arraystretch}{0.4}\textbf{\begin{tabular}[c]{@{}c@{}}GPT-4\\ \tiny \cite{feng2024evaluation}\end{tabular}}

\begin{tabular}{lcllcccccc}
\hline
\multirow{3}{*}{\textbf{Task}} & \multirow{3}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Evaluation\\ Metric\end{tabular}}} & \multirow{3}{*}{\textbf{Dataset}} & \multirow{3}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}\# test \\ ins-\\tances\end{tabular}}} & \textbf{In-domain} & \multicolumn{5}{|c}{\textbf{Generalized LLMs with zero- or few-shot ICL}} \\ \cline{5-10} 
 &  &  &  & \multicolumn{1}{c|}{\multirow{2}{*}{\renewcommand{\arraystretch}{0.4}\textbf{\begin{tabular}[c]{@{}c@{}}BERT-FT\\ \tiny \cite{peng2019transfer} \\ \tiny \cite{gu2021domain} \end{tabular}}}} & \multirow{2}{*}{\renewcommand{\arraystretch}{0.4}\textbf{\begin{tabular}[c]{@{}c@{}}Chat\\-GPT \\\tiny \cite{chen2023extensive}\end{tabular}}} & \multicolumn{1}{c|}{\multirow{2}{*}{\renewcommand{\arraystretch}{0.4}\textbf{\begin{tabular}[c]{@{}c@{}}GPT-4\\ \tiny \cite{feng2024evaluation}\end{tabular}}}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Llama\\ -3-8B\end{tabular}}} & \multicolumn{2}{c}{\textbf{BioMistral}} \\ \cline{9-10} 
 &  &  &  & \multicolumn{1}{c|}{} &  & \multicolumn{1}{c|}{} &  & \textbf{Baseline} & \textbf{Ours} \\ \hline
\multirow{6}{*}{NER} & \multirow{5}{*}{\begin{tabular}[c]{@{}c@{}}Entity-\\ level F1\end{tabular}} & BC2GM^{\dagger} & 6,322 & \multicolumn{1}{c|}{84.5} & 37.5 & \multicolumn{1}{c|}{54.6} & 12.6 & 34.1 &  \underline{\textbf{61.5}} \\ \cline{3-3}
 &  & BC5-chemical^{\dagger*} & 5,385 & \multicolumn{1}{c|}{93.3} & 60.3 & \multicolumn{1}{c|}{78.2} & 52.5 & 45.0 &  \underline{\textbf{89.9}} \\ \cline{3-3}
 &  & BC5-disease^{\dagger*} & 4,424 & \multicolumn{1}{c|}{85.6} & 51.8 & \multicolumn{1}{c|}{63.9} & 38.7 & 33.7 &  \underline{\textbf{67.0}} \\ \cline{3-3}
 &  & NCBI-disease^{\dagger} & 955 & \multicolumn{1}{c|}{89.1} & 50.5 & \multicolumn{1}{c|}{66.0} & 33.5 & 39.9 & \textbf{61.8} \\ \cline{3-3}
 &  & JNLPBA^{\dagger} & 8,657 & \multicolumn{1}{c|}{79.1} & 41.3 & \multicolumn{1}{c|}{45.4} & 33.3 & 25.6 &  \underline{\textbf{64.4}} \\ \cline{2-3}
 & \begin{tabular}[c]{@{}c@{}}Token-\\ level F1\end{tabular} & EBM PICO^{\dagger} & 24,474 & \multicolumn{1}{c|}{73.4} & 55.6 & \multicolumn{1}{c|}{33.5} & 20.2 & 19.6 & \textbf{55.3} \\ \cline{1-3}
DC & F1 & HoC^{\dagger*} & 315 & \multicolumn{1}{c|}{81.5} & 51.2 & \multicolumn{1}{c|}{62.5} & 23.1 & 47.3 &  \underline{\textbf{63.8}} \\ \cline{1-3}
\multirow{2}{*}{QA} & \multirow{2}{*}{Acc} & PubMedQA^{\dagger} & 500 & \multicolumn{1}{c|}{60.2} & 76.5 & \multicolumn{1}{c|}{70.6} & 71.0 & \textbf{72.0} & 70.2 \\ \cline{3-3}
 &  & BioASQ^{\dagger} & 263 & \multicolumn{1}{c|}{94.8} & 88.6 & \multicolumn{1}{c|}{85.7} & 78.7 & 74.9 & \textbf{86.7} \\ \cline{1-3}
\multirow{4}{*}{RE} & \multirow{4}{*}{F1} & GAD^{\dagger} & 534 & \multicolumn{1}{c|}{84.0} & 52.4 & \multicolumn{1}{c|}{51.5} & 55.6 & 55.0 &  \underline{\textbf{58.5}} \\ \cline{3-3}
 &  & DDI^{\dagger*} & 5,761 & \multicolumn{1}{c|}{82.4} & 51.6 & \multicolumn{1}{c|}{37.7} & \textbf{13.2} & 10.0 & 13.0 \\ \cline{3-3}
 &  & ChemProt^{\dagger*} & 14,744 & \multicolumn{1}{c|}{77.2} & 34.2 & \multicolumn{1}{c|}{37.6} & 35.2 & 28.6 &  \underline{\textbf{38.1}} \\ \cline{3-3}
 &  & i2b2-2010^* & 6,292 & \multicolumn{1}{c|}{76.4} & - & \multicolumn{1}{c|}{-} & 38.9 & 30.9 & \textbf{41.8} \\ \cline{1-3}
NLI & Acc & MedNLI^* & 1,422 & \multicolumn{1}{c|}{73.5} & - & \multicolumn{1}{c|}{-} & 49.1 & 49.3 & \textbf{57.5} \\ \cline{1-3}
STS & \begin{tabular}[c]{@{}c@{}}Pearson\\ Corr\end{tabular} & BioSSES^{\dagger*} & 20 & \multicolumn{1}{c|}{92.3} & 42.8 & \multicolumn{1}{c|}{89.3} & 67.9 & 69.1 & \textbf{80.8} \\ \hline
\multirow{2}{*}{Overall} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Macro\\ average\end{tabular}} & BLURB^{\dagger} & - & \multicolumn{1}{c|}{82.9} & 53.4 & \multicolumn{1}{c|}{59.7} & 41.2 & 42.7 &  \underline{\textbf{62.4}} \\ \cline{3-3}
 &  & BLUE$^*$ & - & \multicolumn{1}{c|}{82.8} & - & \multicolumn{1}{c|}{-} & 39.8 & 39.2 & \textbf{56.5} \\ \hline
\end{tabular}
}
\setlength{\belowcaptionskip}{-5pt}
\caption{Our proposed system, BioMistral-NLU's zero-shot performance on 15 unseen medical NLU datasets from 2 benchmarks: BLURB (labeled by $^\dagger$) and BLUE (labeled by $^*$). \textbf{Bold} indicates superior performance over other open-source LLMs, which utilize the same, dataset-agnostic prompts as BioMistral-NLU, under the zero-shot setting, except for two extra random examples for NER tasks. \underline{Underline} indicates better performance over  ChatGPT one-shot and GPT-4 three-shot ICL. ChatGPT and GPT-4 utilize dataset-specific prompts and few-shot examples, and therefore have advantages over our proposed system. `-' indicates that the performance is not measured by prior research. }


\label{tab:results}
\end{table}
